PSDF Fusion: Probabilistic Signed Distance Function for On-the-fly 3D Data Fusion and Scene Reconstruction

We propose a novel 3D spatial representation for data fusion and scene reconstruction. Probabilistic Signed Distance Function (Probabilistic SDF, PSDF) is proposed to depict uncertainties in the 3D space. It is modeled by a joint distribution describing SDF value and its inlier probability, reflecting input data quality and surface geometry. A hybrid data structure involving voxel, surfel, and mesh is designed to fully exploit the advantages of various prevalent 3D representations. Connected by PSDF, these components reasonably cooperate in a consistent frame- work. Given sequential depth measurements, PSDF can be incrementally refined with less ad hoc parametric Bayesian updating. Supported by PSDF and the efficient 3D data representation, high-quality surfaces can be extracted on-the-fly, and in return contribute to reliable data fu- sion using the geometry information. Experiments demonstrate that our system reconstructs scenes with higher model quality and lower redundancy, and runs faster than existing online mesh generation systems.

==> tex/macro.tex <==
% =========================================
% 	Packages
% =========================================
%\usepackage{mathptmx}
\usepackage{times}
\usepackage{epsfig}
\usepackage{xspace}
\usepackage{color}
\usepackage{multirow}
\usepackage{graphics}
\usepackage{adjustbox}
\usepackage{subfigure}
\usepackage{amsmath}
\usepackage[noend]{algpseudocode}
\usepackage{algorithmicx,algorithm}
\usepackage{paralist} % compactitem, compactenum
\usepackage{enumitem}
\usepackage{graphicx} %use graph format
\usepackage{epstopdf}% adjust enum margin
%\graphicspath{{figure/}}
\usepackage{booktabs} % Publication quality tables


\usepackage[pagebackref=true,breaklinks=true,letterpaper=true,colorlinks,citecolor=blue,linkcolor=blue,bookmarks=false]{hyperref}

% =========================================
% 	Macros
% =========================================
%%% short-hand notations
\newcommand{\Paragraph}[1]{\noindent\paragraph{#1}} % avoid indent for paragraph title
\newcommand{\ul}[1]{\underline{\smash{#1}}}
\newcommand{\tb}[1]{\textbf{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\TODO}{{\textbf{\color{red}[TODO]\,}}}
\newcommand{\n}{\vskip\baselineskip}
\def\ith{i^\textit{th}}

%%% comments
\newcommand {\minghsuan}[1]{{\color{red}\bf{Ming-Hsuan: }#1}\normalfont}
\newcommand {\jason}[1]{{\color{magenta}\textbf{Jason: }#1}\normalfont}
\newcommand {\jiabin}[1]{{\color{blue}\textbf{Jia-Bin: }#1}\normalfont}

%%% ignore paragraph
\long\def\ignorethis#1{}

%%% color
\definecolor{Gray}{rgb}{0.35,0.35,0.35}
\definecolor{Blue}{rgb}{0,0.2,0.8}
\definecolor{Red}{rgb}{0.8,0.2,0}
\definecolor{Green}{rgb}{0.0,0.5,0.1}
\definecolor{Gray}{rgb}{0.4,0.4,0.4}
\def\newtext#1{\textcolor{Blue}{#1}}
\def\torevise#1{\textcolor{Red}{#1}}
%\def\modtext#1{#1} % temporary used for submission
\def\red#1{\textcolor{Red}{#1}}
\def\blue#1{\textcolor{Blue}{#1}}
\def\green#1{\textcolor{Green}{#1}}

%%% adjust margin
\newlength\paramargin
\newlength\figmargin
\newlength\secmargin

\setlength{\paramargin}{-1.0mm}
\setlength{\figmargin}{-1.5mm}
\setlength{\secmargin}{-2.5mm}


%% table control
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}


%% Latin abbreviations
\def\ie{i.e.,~}
\def\eg{e.g.,~}
\def\etc{etc}
\def\cf{cf.~}
\def\viz{viz.~}
\def\vs{vs.~}
\def\etal{et~al.\xspace}
\def\Naive{Na\"{\i}ve~}
\def\naive{na\"{\i}ve~}


% symbols using in math
%\DeclareMathOperator*{\argmin}{\arg\!\min}
%\DeclareMathOperator*{\argmax}{\arg\!\max}

\setlength{\fboxsep}{0pt}
\def\padg{{\color{white}g}}

\newcommand{\jbox}[2]{
  \fbox{%
  	\begin{minipage}{#1}%
  		\hfill\vspace{#2}%
  	\end{minipage}%
  }}

\newcommand{\jblock}[2]{%
	\begin{minipage}[t]{#1}\vspace{0cm}\centering%
	#2%
	\end{minipage}%
	}

%% reference macro
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\eqnref}[1]{\eqref{eq:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\prgref}[1]{Program~\ref{#1}}
%\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\clmref}[1]{Claim~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\ptyref}[1]{Property~\ref{#1}}



\newcommand{\dummyfig}[1]{
	\centering
	\fbox{
		\begin{minipage}[c][0.33\textheight][c]{0.5\textwidth}
			\centering{#1}
		\end{minipage}
	}
}
\graphicspath{{figure/eps/}}



==> tex/related-work-backup.tex <==

\section{Related Work}
\noindent \textbf{Volumetric data fusion.}
It is an intuitive idea to divide the world into cells and fit input data into spatially organized positions. It is, however, not trivial to design a function over such discretized space with reliable fusion or inference computations. Generally occupancy probability and signed distance function (SDF) are mostly used.

Elfes \cite{elfes1989using} first introduced 2D occupancy grids in robotics. Afterwards this method has been extended to 3D with many mature off-the-shelf solutions such as OctoMap \cite{Hornung:2013gt} and the 3D version of Cartography \cite{hess2016real}. Utilizing inverse models that assume independencies between voxels, these approaches are mainly designed for real-time large-scale robot navigation and mapping instead of accurate surface reconstruction. To generate refined surfaces within occupancy grids, visual consistency has been used. Woodford \etal \cite{Woodford:2012ee} proposed a joint distribution of point occupancy and outlier ratio with visual constraints and achieved competitive results. Ulusoy \etal \cite{ulusoy2015towards,Ulusoy:CVPR:2016} similarly emphasized ray-consistency to reconstruct global-consistent surfaces, whose inference is sophisticated and cannot run in real-time. Although surface extraction could be performed on occupancy grids via thresholding or ray-casting, it is usually very sensitive to parameters.

Instead of maintaining a $\{0, 1\}$ field, Curless and Levoy \cite{Curless1996} proposed SDF which holds the signed projective distance from voxels to their closest surfaces sampled by input points. This representation has been proved by Newcombe \etal \cite{Newcombe2011} to be extremely suitable for data fusion from modern consumer-level depth sensors. Later on many efforts \cite{Zeng2013,whelan2012kintinuous,Niessner2013,kahler2016hierarchical} have been made to improve the memory efficiency of the data structure using Octrees, moving blocks, hash tables, and hierarchical hash tables. In common, these methods rely on weighted average to fuse data and smooth out noises. As for possibly integrated outliers, Nie{\ss}ner \etal \cite{Niessner2013} used an ad hoc temporal recycle strategy in their implementation; Klingensmith \etal \cite{Klingensmith2015} cut out noisy input by a simple carving. Dai \etal \cite{dai2017bundlefusion} used a weighted subtraction to de-integrate data which are assumed to be incorrectly registered. As a non-local prior, Dzitsiuk \etal \cite{Dzitsiuk2017} refined SDF value on-the-fly using plane fitting, which performs well mainly in flat scenes with relatively low voxel resolutions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{Surfel and point based fusion.}
Surfel and point-based fusion are usually used for sparse or semi-dense reconstructions in SLAM systems using monocular or stereo cameras. Within such data, noises and outliers are inevitable and have to be handled properly during fusion. Vogiatzis \etal \cite{vogiatzis2011video} proposed an elegant math model treating outlier ratio and depth of a point as random variables subject to a special distribution. The parameters of such distributions are updated in a Bayesian fashion. This approach was adopted by Forster \etal \cite{forster2014svo} in SLAM systems with inverse depths, achieving competitive results. 

An alternative is to select ad hoc weights involving geometry and photometric properties of estimated points and computing weighted average\cite{tanskanen2013live,Kolev2014}. This simple strategy shares some similarity to the fusion of SDF values, and is also used in RGB-D systems where depths are more reliable\cite{Keller2013,InfiniTAM_V3_Report_2017}.

%%%%%%%%%%%%%%%%%%%%%%%
\noindent \textbf{On-the-fly mesh generation.}
In an online reconstruction system, there are studies that directly fuse data into mesh. Marton \etal \cite{Marton2009} resampled point clouds spatially managed by KD-Tress, whose computation is not efficient enough. Zienkiewicz \etal \cite{Zienkiewicz2016} generated structured triangles by solving a large sparse linear equation. Maintained as a 2.5D map, the approach is not able to handle occlusions in complex scenes.
Online mesh generation from volumes, whose cornerstone was laid by MarchingCubes proposed by Lorensen and Cline \cite{Lorensen1987} and refined by several following studies \cite{newman2006survey}, has gained its popularity along with the wide use of SDF in dense reconstruction. Steinbrucker \etal \cite{Steinbrucker2014} maintained an octree-based structure where boundary conditions have to be carefully considered. Klingensmith \etal \cite{Klingensmith2015} used spatial hashed blocks and maintained mesh triangles in the block level. Although it is memory efficient for volumes using spatial-hashing techniques, it fails to consider vertex sharing between triangles. Dong \etal \cite{Wei2018} revealed the correspondences between mesh vertices and voxel edges, reducing the redundancy in the aspect of data structure, yet improvement is required to remove false surfaces generated from noisy TSDF voxels.

==> tex/table_statistics.tex <==
\begin{table*}
	\begin{center}
		\resizebox{\textwidth}{!}{
			\begin{tabular}{|l|c||c|c|c|c|c||c|c|}
				\hline
				\multirow{3}{*}{Dataset} &
				\multirow{3}{*}{Frames} &
				\multicolumn{5}{c||}{TIME (ms)} &
				\multicolumn{2}{c|}{MEMORY (vertex count)} \\
				\cline{3-9}
				& & \multicolumn{2}{c|}{Simple} &\multicolumn{2}{c|}{Proposed} & \multirow{2}{*}{Ray-casting}
				& \multirow{2}{*}{Simple} & \multirow{2}{*}{Proposed} \\
				\cline{3-6}
				& & Mapping & Meshing & Mapping & Meshing & & & \\
				\hline\hline
				Zhou/copyroom & 5490  & 0.73 & 38.29 & 1.02 & \textbf{24.52} & 18.95  & 2734581 & \textbf{1393653} \\
				Zhou/lounge & 3000 & 0.88 & 44.82 & 1.29 & \textbf{24.20} & 19.61  & 2739152 & \textbf{1244321} \\
				Zhou/burghers & 11230 & 0.87 & 46.63 & 1.30 & \textbf{25.88} & 25.38  & 1846667 & \textbf{858493} \\
				ICL/lv1 & 965  & \textbf{1.15} & 85.61 & 2.07 & \textbf{49.73} & 26.42  & 2383400 & \textbf{1177154} \\
				ICL/lv2 & 880 & \textbf{1.25} & 113.40 & 2.35 & \textbf{59.32} & 28.59  & 3200191 & \textbf{1486725} \\
				ICL/office1 & 965 & \textbf{1.28} & 79.89 & 2.28 & \textbf{45.56} & 27.48  & 3175945 & \textbf{1516511} \\
				ICL/office2 & 880 & \textbf{1.30} & 97.62 & 2.45 & \textbf{57.46} & 30.22  & 3747019 & \textbf{1751466} \\
				TUM1/freiburg1 & 790  & \textbf{0.75} & 73.03 & 1.20 & \textbf{35.59} & 17.34 & 841405 & \textbf{298543} \\
				TUM2/freiburg2 & 3615 & \textbf{0.97} & 158.98 & 2.05 & \textbf{75.23} & 23.22  & 1154702 & \textbf{386612} \\
				TUM3/freiburg3 & 2486 & \textbf{1.03} & 183.35 & 2.68 & \textbf{105.95} & 24.85  & 2012154 & \textbf{966587} \\
				\hline
			\end{tabular}
		}
	\end{center}
	\caption{Average running time and total vertex consumption of {\it baseline, \it simple}, and {\it proposed} approaches. Our proposed data structure could significantly reduce number of vertices in mesh, even with classical TSDF fusion. Using PSDF, the mesh size could be further constrained with the running speed improved.}\label{tab:table}
\end{table*}
